QUOTAS: A new research platform for the data-driven investigation of black holes

We present QUOTAS, a novel research platform for the data-driven investigation of super-massive black hole (SMBH) populations. While SMBH data sets -- observations and simulations -- have grown rapidly in complexity and abundance, our computational environments and analysis tools have not matured commensurately to exhaust opportunities for discovery. Motivated to explore BH host galaxy and the parent dark matter halo connection, in this pilot version of QUOTAS, we assemble and co-locate the high-redshift, luminous quasar population at $z \geq 3$ alongside simulated data of the same epochs. Leveraging machine learning algorithms (ML) we expand simulation volumes that successfully replicate halo populations beyond the training set. Training ML on the Illustris-TNG300 simulation that includes baryonic physics, we populate the larger LEGACY Expanse dark matter-only box with quasars. Our first science results comparing observational and ML simulated quasars at $z \sim 3$, reveal that while the recovered Black Hole Mass Functions and clustering are in good agreement, simulated SMBHs fail to accrete, shine and grow at high enough rates to match observed quasars. We conclude that sub-grid models of mass accretion and SMBH feedback implemented in Illustris-TNG300 do not reproduce their observed mass growth. QUOTAS, demonstrates the power of ML, both for analyzing large complex datasets, and offering a unique opportunity to interrogate our theoretical model assumptions. We deploy ML again to derive and devise an optimal survey strategy for bringing the undetected lower luminosity quasar population into view. QUOTAS, and all related materials are publicly available at the Google Kaggle platform.

==> styles.tex <==
% Style definitions 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}

%\bibliographystyle{elsarticle-num}

==> tables.tex <==


\def
\tablebh
{
\begin{table*}
\centering
\begin{tabular}{ccccc}
\hline 
$z$ Range & Num. Quasars & Luminosity Estimator & Vel. Disp. Estim. & Reference  \\
\hline
3.01-4.33 & 43 & \begin{tabular}{@{}c@{}} $L_{\lambda}(1350)$, $L_{\lambda}(3000)$, \\ $L_{\lambda}(5100)$, $L(H\beta)$, $L(MgII)$ \end{tabular},& $H\beta$, Mg II, C IV  & \cite{2019ApJS..241...34S} \\
3.00-5.46 & 7955 & \begin{tabular}{@{}c@{}} $L_{\lambda}(1350)$, $L_{\lambda}(3000)$, \\ $L_{\lambda}(5100)$, $L(H\beta)$, $L(MgII)$ \end{tabular} & H$\beta$, Mg II, C IV & \cite{2011ApJS..194...45S} \\
3.00-4.89 & 26571 & $L_{\lambda}(1350), L_{\lambda}(3000), L_{\lambda}(5100)$ & Mg II, C IV &\cite{2017ApJS..228....9K} \\
3.22-3.76 & 24 & $ L_{\lambda}(3000), L_{\lambda}(5100)$ & H$\beta$, Mg II & \cite{2015ApJ...799..189Z} \\
4.52-6.41 & 21 & $L_{\lambda}(3000)$ & Mg II & \cite{2011ApJ...739...56D} \\
4.66-4.92 & 40 & $L_{\lambda}(1450), L_{\lambda}(3000) $ & Mg II    & \cite{2011ApJ...730....7T} \\
5.64-6.42 & 50 & $L_{\lambda}(1350),  L_{\lambda}(1700), L_{\lambda}(3000)$ & Mg II, CIV & \cite{2019ApJ...873...35S} \\
5.77-6.31 & 6  & $L_{\lambda}(1350),  L_{\lambda}(3000)$ & Mg II, CIV & \cite{2007AJ....134.1150J} \\
5.82-6.28 & 5  & $L_{\lambda}(1350),  L_{\lambda}(3000)$ & Mg II, CIV & \cite{2007ApJ...669...32K} \\
5.90      & 1  & $L_{\lambda}(3000)$ & Mg II & \cite{2018ApJ...867...30E} \\
5.98-6.44 & 9  & $L_{\lambda}(3000)$ & Mg II & \cite{2010AJ....140..546W} \\
6.13      & 1  & $L_{\lambda}(3000)$ & Mg II & \cite{2017ApJ...845..138S} \\
6.48-7.08 & 11 & $L_{\lambda}(3000)$ & Mg II & \cite{2017ApJ...849...91M} \\
6.60-7.10 & 4  & $L_{\lambda}(3000)$ & Mg II, CIV & \cite{2014ApJ...790..145D} \\
7.07      & 1  & $L_{\lambda}(1350)$ & Mg II & \cite{2019ApJ...872L...2M} \\
\hline 
\end{tabular}
\caption{The compiled list of quasars including additional properties of the supermassive black holes included in our database. This table comprises data from reported spectroscopic measurements of individual quasars.
\label{tab:bh_prop_samples}}
\end{table*}
}



\def
\tableqsosurvey
{
\begin{table*}
  \centering
  \begin{tabular}{cllrr}
  %\begin{tabular}{cllrS}
    \hline
    $z$ range & Survey & Reference & Number & {Area} \\
    & & & of quasars & {(deg$^2$)} \\
    \hline
    2.2--3.5 & BOSS DR9 & \cite{2013ApJ...773...14R} & 23301 & 2236.0 \\
    3.7--4.7 & SDSS DR7 & \cite{2010AJ....139.2360S} & 1785 & 6248.0 \\
    3.6--5.2 & NDWFS & \cite{2011ApJ...728L..26G} & 12 & 1.71 \\
    3.8--5.3 & DLS & \cite{2011ApJ...728L..26G} & 12 & 2.05 \\
    4.7--5.4 & SDSS+WISE & \cite{2016ApJ...829...33Y} & 99 & 14555.0 \\
    4.7--5.5 & SDSS DR7 & \cite{2013ApJ...768..105M} & 103 & 6248.0 \\
    4.7--5.5 & --- Stripe 82 & \cite{2013ApJ...768..105M} & 59 & 235.0 \\
    5.7--6.5 & SDSS Main & \cite{2016ApJ...833..222J} & 24 & 11240.0 \\
    5.7--6.5 & --- Overlap & \cite{2016ApJ...833..222J} & 10 & 4223.0 \\
    5.7--6.5 & --- Stripe 82 & \cite{2016ApJ...833..222J} & 13 & 277.0 \\
    5.8--6.6 & CFHQS Deep & \cite{2010AJ....139..906W} & 1 & 4.47 \\
    5.8--6.6 & --- Very Wide & \cite{2010AJ....139..906W} & 16 & 494.0 \\
    5.8--6.5 & Subaru High-$z$ Quasar & \cite{2015ApJ...798...28K} & 2 & 6.5 \\
    4.0--6.5 & CANDELS GOODS-S & \cite{2015AA...578A..83G} & 19 & 0.047 \\
    6.5--7.4 & UKIDSS & \cite{2011Natur.474..616M} & 1 & 3370.0 \\
    6.5--7.4 & UKIDSS & \cite{2015ApJ...801L..11V} & 1 & 3370.0 \\
    6.5--7.4 & \begin{tabular}{@{}c@{}}ALLWISE+UKIDSS \\ +DECaLS\end{tabular} & \cite{2018Natur.553..473B} & 1 & 2500.0 \\
    \hline
  \end{tabular}\\
  \caption{
  The list of quasar survey samples that are included in our database and QuasarNet research portal.
    \label{tab:qlf_samples}
}
\end{table*}
}


\def
\tabledm
{
\begin{table*}
  \centering
  \begin{tabular}{ccc}
  \hline
    Name & Units & Description \\
  \hline
    $z$                 & -             & redshift \\
    $M_{\rm{vir}}$      & $M_{\odot}$   & virial mass \\
    $r_{\rm{vir}} $     & kpc           & virial radius \\
    $x, ~y, ~z$         & Mpc           & position \\
    $v_x, ~v_y, ~v_z$   & $\rm{km ~ s^{-1}}$      & peculiar velocity \\
    $ J_x, ~J_y, ~J_z$  & $M_{\odot}$ Mpc $\rm{km ~ s^{-1}}$  & angular momentum \\
    $ \dot{M}_{\rm{acc}}$ & $M_{\odot}/$yr & accretion rate onto halo \\
    $I_{\rm{desc}} $ & - & descendant halo ID \\
    $T/|U|$ & - & virial parameter \\
    $x_i, ~y_i, ~z_i$         & Mpc           & position of each particle \\
    $v_{x,i}, ~v_{y,i}, ~v_{z,i}$   & $\rm{km ~ s^{-1}}$     & peculiar velocity of each particle \\
   \hline
  \end{tabular}\\
  \caption{
  Examples of dark matter halo properties stored in the database.
  \label{table:dm_halo_properties}
  }
\end{table*}
}


